R&F-Inventory: A Large-Scale Dataset for Monotonic Inventory Estimation in Reach and Frequency Advertising

Reach and Frequency (R&F) contract advertising is an important form of widely used brand advertising. Unlike performance advertising, R&F contracts emphasize controllable delivery of UV and PV under given targeting, scheduling, and frequency control constraints. In practical systems, advertisers typically need to view the UV, PV change curves at different budget levels in real time when creating an R&F contract. However, most existing publicly available advertising datasets are based on independent samples, lacking a characterization of the core structure of the "budget-performance curve" (including UV and PV) in R&F contracts.This paper proposes and releases a large-scale R&F contract inventory estimation dataset. This dataset uses the R&F contract context consisting of "targeting-scheduling-frequency control" as the basic context, providing observations of UV and PV corresponding to multiple budget points within the same context, thus forming a complete budget-performance curve. The dataset explicitly includes a time-window-based frequency control mechanism (e.g.,"no more than 3 times within 5 days") and naturally satisfies the monotonicity and diminishing marginal returns characteristics in the budget and scheduling dimensions. We further derive the theoretical maximum exposure ceiling and use it as a consistency check to evaluate data quality and the feasibility of model predictions. Using this data set, this paper defines two standardized benchmark tasks: single-point performance prediction and reconstruction of budget-performance curves, and provides a set of reproducible baseline methods and evaluation protocols. This dataset can support systematic research on problems such as structural constraint learning, monotonic regression, curve consistency modeling, and R&F contract planning.The code for our experiments can be found at https://github.com/pengyunshan/RF-Inventory.

==> 2.pre.tex <==
\subsection{Online Advertising Bidding as a Sequential Decision Problem}
\label{subsec:bidding}
We consider an online advertising bidding system operating in a real-time auction environment. Time is discretized into decision windows of fixed length (e.g., two minutes), which aligns with practical bidding systems where bid adjustments are performed at coarse temporal granularity rather than per PV.
At each decision window t, the system observes the current environment state  $s_t$
, selects a bidding strategy, and receives feedback aggregated over the window. The goal of the system is to maximize long-term cumulative value under budget and pacing constraints.
\begin{align}
\begin{aligned}
    \label{eq:1}
    \max \sum_{j} \mathbb{A}_{ij} \cdot v_{ij} \quad s.t. \sum_{j} (\mathbb{A}_{ij} \cdot b_j) &\leq B_i,\\
    \frac{\sum_{j} (\mathbb{A}_{ij} \cdot \mathbb{P}_{ij})}{\sum_{j} (\mathbb{A}_{ij} \cdot v_{ij})} &\leq C_{i}.
\end{aligned}
\end{align}

Where $B_i$ represents the advertiser's budget; $C_i$ represents the ad's ROI constraint; $A_{ij}$ indicates whether the ad wins the bid, $b_j$ represents the cost of winning the bid; $v_{ij}$ indicates whether a conversion actually occurred after winning the bid; and $P_{ij}$ indicates the cost of winning the bid and gaining exposure.


\subsection{agentHPO}

In recent years, Large Language Models (LLMs) have been introduced into the field of Hyperparameter Optimization (HPO) to replace traditional parameter tuning methods based on heuristic rules or black-box search. Unlike numerical search problems that treat parameter optimization as independent trials, related work models it as a sequential decision-making process based on historical experimental information. In this process, the LLM acts as an agent, iteratively generating new parameter adjustment strategies based on past parameter configurations and performance feedback. This type of method is often called Agent-based HPO (AgentHPO). Its advantages lie in its ability to comprehensively utilize prior knowledge, experimental logs, and training state information, flexibly supporting high-dimensional mixed parameter spaces, dynamic search strategies, and multi-objective constraints, providing a unified and scalable modeling paradigm for parameter optimization of complex models and systems.

\subsection{On-Policy Reinforcement Learning and SARSA}
To achieve adaptive model selection while maintaining safety, we employ a policy-based reinforcement learning approach at the model selection level.

SARSA (State-Action-Reward-State-Action) is a policy-based temporal differential control algorithm that learns the action-value function $π(s,a)$ under the current action policy π. Given a transition $( α , β , α , α , α , α + 1 , β + 1 )$, SARSA updates the action value estimate as:

$α ( α(α, β(α)) ← α(α(α, β(α)) + α[β(α) + α α(α(α+1, β(α+1)) − α(α(α, β(α))]$,

where α Let be the learning rate, +1), sampled from the same policy used for action selection.

Unlike off-policy methods guided by a greedy objective policy, SARSA evaluates the value of actual actions taken, making it particularly suitable for environments where exploration itself affects system dynamics. Safety.

In our setting, the SARSA agent operates at the model selection level. The action-value function Q(s,a) represents the expected long-term utility of choosing bidding expert a in state s, given the current exploration policy. At each decision window, the agent:
Observes the current state $s_t$, selects bidding expert $a_t$ according to the in-policy exploration policy (e.g., ε-greedy or softmax), executes the selected expert throughout the window, observes the aggregate reward $r_t$, and the next state $s_{t+1}$, samples the next action as $a_{t+1}$, and updates the action-value function via SARSA.

By limiting online learning to a discrete set of safe experts, the system achieves controlled exploration while avoiding direct manipulation of bidding prices.

